On-the-Job Learning with Bayesian Decision Theory

Our goal is to deploy a high-accuracy system starting with zero training examples. We consider an "on-the-job" setting, where as inputs arrive, we use real-time crowdsourcing to resolve uncertainty where needed and output our prediction when confident. As the model improves over time, the reliance on crowdsourcing queries decreases. We cast our setting as a stochastic game based on Bayesian decision theory, which allows us to balance latency, cost, and accuracy objectives in a principled way. Computing the optimal policy is intractable, so we develop an approximation based on Monte Carlo Tree Search. We tested our approach on three datasets---named-entity recognition, sentiment classification, and image classification. On the NER task we obtained more than an order of magnitude reduction in cost compared to full human annotation, while boosting performance relative to the expert provided labels. We also achieve a 8% F1 improvement over having a single human label the whole set, and a 28% F1 improvement over online learning.

==> bounds.tex <==
\section{Theoretical Bounds on Active Classification Performance}
\label{sec:bounds}

We're interested in providing extreme limits of classifier performance under an unrealistic set of assumptions, as a way to gain intuition about the setting and the limitations of our approach.
It's trivially easy to see that it is possible to spend no money, and no time, during classifications. Simply return null on every request.
It's more interesting to evaluate if it's possible to return a perfect classification every time, and how much we have to give up in average cost to achieve perfection.
Let's assume that our temporal and financial budgets are infinite, we have an infinite number of humans on call, and we have an accurate model of the confusion matrix of humans $C$.
If all of these conditions are met, are there any guarantees we can make about our classifier?
Trivially, if our classifier always returns a uniform distribution over all possible output labels, and we query an infinite number of humans, it is possible to achieve arbitrary accuracy.
More interestingly, are there non-trivial bounds we can set on the cost-guarantee tradeoffs?

As an overview, our analysis will first define the value of valid priors on the data in terms of number of human queries required, under some simplifying assumptions about human error.
We will then focus on the challenge of not being able to absolutely trust model confidence estimates.
We define a rigorous way of conceptualizing ``trust'' in our confidence values, which requires defining the set of ``true confidence'' estimates allowable by the data for a given input.
Then we define bounds of expected classification performance given a choice for this ``trust,'' and demonstrate that more trust leads to higher error rates and lower costs.

\subsection{True Confidence Values}

First we must define the set of ``true confidence'' distributions $\Delta$.
Let data arrive in the form of $(\bx_i,\by_i)$ pairs, where $\by_i$ is the always observed set of variables we condition on, and $\bx_i$ is the true observed outcome.
Given a set $\Gamma$ of IID pairs, a norm $N$, and a feature mapping $f(\by) = \bz \in \sR^m$,
 let the ``$\epsilon$-neighborhood'' of $\by_t$ (notation $\Gamma(\epsilon, \by_t)$) be defined as all pairs in $\Gamma$ within the norm ball under $N$ of size $\epsilon$:
\[\Gamma(\epsilon, \by_t) = \{\bx_i \in \Gamma | ||f(\by_i) - f(\by_t)||_N \leq \epsilon\}\]
Every $\epsilon$-neighborhood, for $\epsilon \in \sR^+$, defines a natural frequentist estimate for $P(\bx_t | \by_t)$:
\[P(\bx_t | \by_t; \epsilon) \approx \sum \frac{\Gamma(\epsilon, \by_t)}{|\Gamma(\epsilon, \by_t)|}\]
Intuitively, $\epsilon$ has two limit conditions:
\[\lim_{\epsilon\to\infty} P(\bx | \by; \epsilon) = \sum \frac{\bx_i}{|\Gamma|}\]
\[\lim_{\epsilon\to0} P(\bx | \by; \epsilon) = \sum \frac{\bx_i | \by_i = \by_t}{\sum \mathbbm{1}\{\by_i = \by_t\}}\]
Let the set of ``true confidence'' distributions $\Delta$ be defined as
\[\Delta = \{P(\bx | \by; \epsilon) | \epsilon \in \sR^+\}\]

\subsection{The Value of Valid Priors}

Assume we are given a vector $\by$, and we want to predict $\bx = \argmax_{\bx} P(\bx | \by)$, and we have access to an infinite number of human labelers, as explained above.
We are tasked with, regardless of cost, ensuring that when given an infinite number of $\by_i$, we achieve an error rate of $e_{\text{acceptable}}$
\[\lim_{i\to\infty} \frac{\sum_i \frac{||\bx_{i,\text{true}} - \bx_{i,\text{guess}}||_{\infty}}{|\bx|}}{i} \leq e_{\text{acceptable}}\]
In practice, this implies the policy of turning in a vector of guesses $x$ only when
\[\min_{i} \max_{k} P(\bx_i = k | \by) > 1 - e_{\text{acceptable}}\]
Until that condition is met, we must continue asking queries of humans.
For simplicity of analysis, to derive a lower bound on value of information, let's assume that we're confined to treating each variable in $\bx$ independently.
As we arrive at a variable $i$, any previous human queries asked of nodes $j < i$ are already incorporated in our observed marginals for $\bx_i$.

Let's assume that our model delivers perfectly accurate marginals $m_i$ for the classes $\bx_i$.
Formally, all marginals $m_i \in \Delta$.
How does a setting of $m_i$ effect expected number of queries to achieve $\min_{i} \max_{k} P(\bx_i = k | \by) > 1 - e_{\text{acceptable}}$?

Let's assume a simplified model of human error for this analysis, where humans are defined as follows:
\begin{equation}
    Q(o_i, X_j) \sim
    \begin{cases}
       \text{uniformly drawn from } D_j = \{1 \ldots K_j\}, & \text{with probability}\ \epsilon \\
      h_{\text{true}}(X_j), & \text{otherwise}
    \end{cases}
\end{equation}

Then we can easily derive that a human query is worth a \todo{math} reduction in expected $E[\min_{i} \max_{k} 1-P(\bx_i = k | \by)]$.
This then leads to the recurrence for expected number of queries remaining given $c$.

\[E[\text{\# queries}] = \text{\todo{recurrance}}\]

\subsection{The Worst-case Cost of Invalid Priors}
\label{sec:worst-case}

Let's assume that our model's prior is not valid ($m_i \not\in \Delta$), but is ``close,'' as in $\min (||M(\by_i, j) - \delta||_N | \delta \in \Delta) < \gamma$, for some $\gamma \in \sR^+$, and norm $N$.
What's the worst that could happen to our accuracy, assuming we're still running the algorithm in the last section (turn in when $\min_{i} \max_{k} P(\bx_i = k | \by) > 1 - e_{\text{acceptable}}$, otherwise query).
We have $m_i \not\in \Delta$ and $m_{i,\text{true}} \in \Delta$ where $m_{i,\text{true}} = argmin_{\delta} (||m_i - \delta||_N, \delta \in \Delta)$.

Given that our humans are drawn from \todo{$H = $humans cross $m_{i,\text{true}}$}, we have that our algorithm will terminate when
\[\max_{k} (m_i \times H^{\text{\# queries}})_k > 1 - e_{\text{acceptable}}\]
This will produce more errors than $e_{\text{acceptable}}$, as described by:
\[g(\gamma) = \text{\todo{math}}\]

\subsection{Trust Guarantees for Model Confidence Estimates}

Given a model $M$ which is capable of providing confidence estimates, we would like to quantify how much trust we can place in these estimates.
Let $M(\by_i, j) = c_j \in R^k$, where $c_j$ is the vector of marginal class probabilities for node $j$ predicted by the model.
Let $\gamma \in R^+$ be constants $\beta \in R^+$, and $N$ be a norm, then we define a trust guarantee for our model to be a statement of $(\gamma, \beta, N)$ where
\[P(\min (||M(\by_i, j) - \delta||_N | \delta \in \Delta) > \gamma) \leq \beta\]
A set of approximate trust guarantees $(\gamma, \beta, N)$ can be estimated in practical contexts by observing $\Delta$ for a finite set of $\epsilon$ on a held out dataset, and calculating directly.
Note that it is possible to produce guarantees that set $\beta = 0$, by simply setting $\gamma = \infty$.
Likewise $\gamma = 0$ is easily achieved with $\beta = \infty$.
These are not useful bounds.

\subsection{Model Under-Confidence}

In practice, $\Delta$ is never observed, so we have to perform some approximations if we want to provide real guarantees.
We know, however, a good estimate of one member of $\Delta$: the underlying class distribution $\delta_{\text{class}} \in \Delta$.
It's intuitive that model underconfidence, in the extreme case always predicting $\delta_{\text{class}}$, yields both $\gamma \approx 0$ and $\beta \approx 0$.
By Chebyshev, assuming some underlying data variance $\sigma$, we have the following guarantees for our massively underconfidence model:
\[\gamma = k\sigma, \beta = \frac{1}{k^2}, \text{for all} k \in \sR\]
In this way we can achieve a tight guarantee, but the information provided by our model is worth very little.

\subsection{$\gamma$-$\beta$ Query-Bound Tradeoffs}

Given a choice of a $(\gamma, \beta, N)$ trust guarantee, how can we describe model performance?

For argument, assume that for now our $\beta = 0$ and $\gamma < \infty$.
Then we can say with certainty that all our $M(\by_i, j) = c_j$ are within $\gamma$ of some true $\delta \in \Delta$.
Assume our target is some $e_{\text{acceptable}}$ error rate, then we can use the formula from \ref{sec:worst-case} to solve for a new $e_{\text{acceptable $\gamma$-adjusted}}$ given $e_{\text{acceptable}}$, given our $\gamma$ guarantee:
\[\text{todo{math}}\]
This results in an expected number of queries, as a function of $e_{\text{acceptable}}$ and $\gamma$.
\[\text{todo{math}}\]

Now consider $\beta > 0$. In the worst case all the instances where our model prediction is worse than $\gamma$, $\min (||M(\by_i, j) - \delta||_N | \delta \in \Delta) > \gamma$, we just get wrong.
That means that our new expected error rate is $e_{\text{acceptable $\gamma$-adjusted}} + \beta$.
We do not attempt any guarantees that get below $\beta$ in expected error rate.

This means that for larger $\gamma$, we can provide an arbitrary expected error rate, at much greater cost in queries, since we know how to compensate correctly for a $\gamma$ error rate.
Larger $\beta$ will allow smaller $\gamma$, and consequently a smaller number of queries, but the floor on our minimum expected error rate is increased.


==> human-error.tex <==
\section{Modeling human error}
\label{sec:human-error}

\pl{should we have this entire section up front;
it seems like you have to talk about human error in the original framework}

Accurately identifying and hence modeling labeling noise is important if we would like to maximize the information we can get from labelers.


\todo{(arun): rewrite}

Our learner will be allowed to query humans for additional certainty about individual random variables (nodes) $X_i$.
 Humans will exist in a pool $\sP$.
 An individual human $o_i \in \sP$ (for ``oracle'', using the loosest possible definition of oracle) has a model for expected behavior.
Our learner will be allowed to query humans for additional certainty about individual random variables (nodes) $X_i$.
 Humans will exist in a pool $\sP$.
 An individual human $o_i \in \sP$ (for ``oracle'', using the loosest possible definition of oracle) has a model for expected behavior. Specifically, we model the $o_i$ expected delay to respond to a question, and the error function (i.e. response given the true state of the world $h_{\text{true}}$).

For this work we use a simplified model of error, shared uniformly across crowd workers.
 Previous work \cite{yan2011active} \cite{donmez2008proactive} \cite{golovin2010near} has shown that in an offline setting treating oracles uniformly leads to a loss, but in practice our pool is churning so quickly that we don't have time to learn accurate distinctions between workers.
 We leave a solution to this problem to future work.

When asked about variable $X_j$, human error is modeled as correct (returns $h_{\text{true}}(X_j)$) with probability $1-\epsilon$, and chosen uniformly at random from $D_j$ with probability $\epsilon$.
 We use the notation $Q(o_i, X_j)$ to denote the response from asking human $i$ about random variable $j$.

\begin{equation}
    Q(o_i, X_j) \sim
    \begin{cases}
       \text{uniformly drawn from } D_j = \{1 \ldots K_j\}, & \text{with probability}\ \epsilon \\
      h_{\text{true}}(X_j), & \text{otherwise}
    \end{cases}
 \end{equation}
 
This answer arrives after a delay.
 We model the amount of time the worker takes to answer with a gaussian, parameterized by $\mu$ and $\sigma$.
 We use the notation $\sD(o_i, X_j)$ to denote the delay in response when asking human $i$ about random variable $j$.

\[\sD(o_i, X_j) \sim \sN(\mu, \sigma^2)\]

This is an imperfect model, since it assigns some mass to a negative response time, which is impossible, but given a large $\mu$ and relatively small $\sigma$ the mass assigned to $\sD(o_i, X_j) < 0$ is negligible, and it otherwise accurately reflects human response times.


==> partial-monitoring.tex <==
\section{Partial Monitoring Game}
\label{sec:partial}

To cast this problem as a Partial Monitoring Game, we must first make sure the outcome space $\sS$ is finite, which requires that we discretize time into epochs of length $t_{\text{epoch}}$, and impose a time limit on the game, $t_{\text{max}}$, resulting in a finite game space $\sS_{\text{discrete}}$.

\todo{details on how Partial Monitoring Games work}

We can define the entries of our loss matrix $L$ with respect to our loss function $\sL(h_{\text{final}}, h, m, t)$.
 The language $\Sigma$ used to populate our observability matrix $H$ is defined as the state space of the game $\sS_{\text{discrete}}$.

\todo{do math... borrow bounds from Bartok et. al, show Pareto optimal policy}

Our goal is to pick a policy $\pi^*$ to minimize the loss in the terminal state of the algorithm $s_{\text{final}}$.
 Since our loss term depends on the true state of the world $\theta^* = (h_{\text{true}}, t, m)$, of which only $t$ and $m$ are ever known, we can't do this directly.
 However, we have a distribution over our beliefs $p(h_{\text{true}})$ at every step (and consequently the state of the true state of the world $\theta^*$, since $t$ and $m$ are known), so we instead minimize \textit{risk}, which is defined with respect to a particular state of the world $\tilde{\theta}$ as
\[E_{\Theta \sim p(\theta)}[Loss(\Theta || \tilde{\theta})] = \int_{\theta} Loss(\theta || \tilde{\theta})p(\theta)d\theta\]

We can formulate our goal in concrete terms as follows:
\begin{equation*}
\begin{aligned}
& \underset{\pi}{\text{minimize}}
& & E_{\pi}[E_{h \sim p(h)}[\sL(h_{\text{final}}, h, m, t)]] \\
%& \text{subject to}
%& & a \in \sA
\end{aligned}
\end{equation*}

This reduces to the Optimal Decision Tree problem, which is NP-hard.



==> related.tex <==
\section{Related Work}
\label{sec:related}

Our work brings together ideas from active learning, active classification and collective intelligence systems (crowdsourcing).
%the active classification and learning literature as well as literature on collective intelligence systems from the human computer interaction community.
%Our focus has been to address the practically relevant questions that arise at the watershed of these two fields: how to optimally classify instances in {\em real-time} allowing {\em queries} to {\em noisy oracles}. 
In this section, we review prior work and situate our own work within the literature.
%We also contrast our system with the popular active learning and active classification literature.

\paragraph{Active learning and classification.}
Active learning\footnote{We refer the readers to~\cite{settles2010active} for a survey of active learning methods and variants.} is a popular approach to minimize the labeled data required to train a classifier. 
Several authors in the active learning community have considered using crowd workers as a noisy oracle~\cite{yan2011active,vijayanarasimhan2014large}.
However, active learning optimizes over the choice of a subset of a pool of unlabeled that minimizes the risk of the classifier obtained by training on that subset. 
In contrast, on-the-job learning does not get to observe unlabeled data, is allowed to query at test time and must minimize the risk of that example (while trading off cost and latency).

Closely related is active classification~\cite{greiner2002learning,chai2004test,esmeir2007anytime} which asks what is the {\em most informative feature\/} to measure at test time.
One could view our measurements as high-informative features, however our work differs in two respects: we never get to actually observe the true labels and our system is evaluated on regret as opposed to classifier risk.
Existing active classification algorithms rely on having a fully labeled dataset which is used to learn when certain features should be queried.

%Settles et al.~\cite{settles2008analysis} compare different utility choices when querying for complete labels for a CRF sequence model.
There is little existing work on querying a subset of the labels within a single structured output problem.
Angeli et al.~\cite{angeli2014combining} identify instances to label within a cluster of examples in a distantly supervised setting. While this choice was a subset of the labels in the graphical model, interactions between other labels in cluster were not considered.
Liang et al.~\cite{liang09measurements} introduced the measurement framework and studied the problem of active selection of measurements in the active learning setting. 
%However, the measurements considered were aggregated across the dataset (e.g.\ the expected proportion of a label), rather than label measurements within an instance.
\pldone{well, within an example in some sense is a special case and the easy part, so you shouldn't use this as the contrast}{hopefully contrasting with active learning is sufficient for measurements?}

%We refer the reader to \cite{settles2010active} for a survey of active learning and its variants.


% This is more of a UI sort of thing, not really useful to us.
%~\cite{roth2006active} and~\cite{culotta2005reducing}, where humans perform top-K selection over model predictions.
%The systems fall back by stages to traditional no-assistance annotation if the top-K doesn't contain the any correct information.

% Ignoring Tong et. al because it's complex and doesn't quite handle this structured thing. It's about sampling for variables conditioned on somethin.
%jit in the context of fully Bayesian networks where the oracle can draw samples conditioned on certain ``controllable'' values - introduce the notion of expected posterior risk - something we also use.


% While this approach is effective when possible, it relies on the model to consistently produce the correct answer in a top-K for some very small $K$, so for large output spaces it breaks down.

%\paragraph{Noisy oracles}
%
%There's been a line of work on Active Learning in the context of multiple noisy, expensive oracles (\cite{donmez2008proactive,golovin2010near,yan2011active,vijayanarasimhan2014large}).
%This work tries to relax the traditional assumptions in active learning that the oracle is infallible and has no economic cost.
%Some of this work is directly motivated by applications to crowd-sourcing platforms that we investigate.
%WHY DIFFERENT?

% Bayesian priors we use not.
%Finally Bayesian active learning (\cite{golovin2010near},~\cite{tong2000active}) allows us to incorporate a Bayesian prior over our data, and we'll use this as a foundation for our approach to solving the asynchronous behavior problem.

\paragraph{Collective intelligence systems.}
Using crowd workers to assist labeling tasks is an area of active research within the HCI community.
\textit{Flock}~\cite{cheng2015flock} first crowdsources the identification of features for an image classification task, and then asks the crowd to annotate examples.
The system learns to classify images using a decision tree based on the features identified by the crowd.
As a consequence, the system always relies on humans to provide features and there is no transfer of knowledge from humans to a machine learning model as in on-the-job training.
In another line of work, \textit{TurKontrol}~\cite{dai2010decision} models individual crowd worker reliability to optimize the number of human votes needed to achieve confident consensus using a POMDP\@.
%We also model the reliability of workers though using an unsupervised model, similar to \findcite{crowd em}.
Finally, recent work has studied how to support real-time behavior with crowd workers~\cite{bernstein2011crowds,lasecki2013real} by hiring workers ``on retainer''.
We use the same retainer model to maintain a pool of real-time crowd workers with low response times.

% Using crowds to power decision making is not a new idea. Systems in this space that support real-time behavior include \textit{Adrenaline}~\cite{bernstein2011crowds} and \textit{Legion AR}~\cite{lasecki2013real}, which both use a system where crowds are recruited ``on-retainer'' in order to be available at a moments notice.
% We use the same retainer model to maintain a pool of real-time workers with low response times.
%Using artificial-intelligence-crowd hybrids for time-insensitive workflows has also been previously explored.
%It makes no effort to train a model to augment or take over from the workers, so costs remain constant over time.
%Empirical studies have shown that this is an effective method for managing complex workflows \cite{peng2011artificial}.
%Our work follows \cite{peng2010decision} in that we apply Decision Theory to the problem of when to query the crowd, but we train a model to take over for the workers over time, and we handle the additional real time response constraint.

\ac{I omitted partial monitoring games because it seems to be covered in the algo section.}
%\paragraph{Partial monitoring games.}
%\noteb{This bullet point is actually to motivate that our problem is theoretically feasible.}
%Our evaluation metric is unique in the active learning space in that consider a loss we do not observe because we never receive true labels.
%By treating the measurements as partial feedback, our work can be theoretically modeled as a partial monitoring game\cite{cesabianchi06regret} and, in particular, an instance of the label-efficient learning problem\cite{cesabianchi05minimizing}.
%Cesa-Bianchi et al.~\cite{cesabianchi06regret} show that in the online setting, the regret of a partial monitoring game is lower bounded by $O(T^{2/3})$, where $T$ is the number of examples seen. They also provide an algorithm that meets this bound: use the current model to pick the best label and query for complete labels at random with a small probability to update your model.
%These guarantees provide theoretical foundation for our work.

% We already discussed expectimin trees in the relevant section.
%\paragraph{Expectimin trees and game playing}
%Monte Carlo based search methods~\cite{browne2012monte} are a common solution for finding a policy for an expectimin tree. 
%Our usage is slightly different in that we do not need to explore infinite depth.
%Monte Carlo tree search can be extended to continuous state spaces using progressive widening.
%However, because so much information is shared across time, we propose a slight modification of the Dyna-2\cite{silver2008sample} algorithm which proposes features for a linear state value function.
%we do not use separate local features because our  
%- Using state has been explored in Dyna-2 - we do not use a separate set of local features because the state space isn't sufficiently different.



==> std-macros.tex <==
% version 1.2 05/21/08
\newcommand\sa{\ensuremath{\mathcal{a}}}
\newcommand\sd{\ensuremath{\mathcal{d}}}
\newcommand\se{\ensuremath{\mathcal{e}}}
\newcommand\sg{\ensuremath{\mathcal{g}}}
\newcommand\sh{\ensuremath{\mathcal{h}}}
\newcommand\seye{\ensuremath{\mathcal{i}}}
\newcommand\sj{\ensuremath{\mathcal{j}}}
\newcommand\sk{\ensuremath{\mathcal{k}}}
\newcommand\sm{\ensuremath{\mathcal{m}}}
\newcommand\sn{\ensuremath{\mathcal{n}}}
\newcommand\so{\ensuremath{\mathcal{o}}}
\newcommand\sq{\ensuremath{\mathcal{q}}}
\newcommand\sr{\ensuremath{\mathcal{r}}}
\newcommand\st{\ensuremath{\mathcal{t}}}
\newcommand\su{\ensuremath{\mathcal{u}}}
\newcommand\sv{\ensuremath{\mathcal{v}}}
\newcommand\sw{\ensuremath{\mathcal{w}}}
\newcommand\sx{\ensuremath{\mathcal{x}}}
\newcommand\sy{\ensuremath{\mathcal{y}}}
\newcommand\sz{\ensuremath{\mathcal{z}}}
\newcommand\sA{\ensuremath{\mathcal{A}}}
\newcommand\sB{\ensuremath{\mathcal{B}}}
\newcommand\sC{\ensuremath{\mathcal{C}}}
\newcommand\sD{\ensuremath{\mathcal{D}}}
\newcommand\sE{\ensuremath{\mathcal{E}}}
\newcommand\sF{\ensuremath{\mathcal{F}}}
\newcommand\sG{\ensuremath{\mathcal{G}}}
\newcommand\sH{\ensuremath{\mathcal{H}}}
\newcommand\sI{\ensuremath{\mathcal{I}}}
\newcommand\sJ{\ensuremath{\mathcal{J}}}
\newcommand\sK{\ensuremath{\mathcal{K}}}
\newcommand\sL{\ensuremath{\mathcal{L}}}
\newcommand\sM{\ensuremath{\mathcal{M}}}
\newcommand\sN{\ensuremath{\mathcal{N}}}
\newcommand\sO{\ensuremath{\mathcal{O}}}
\newcommand\sP{\ensuremath{\mathcal{P}}}
\newcommand\sQ{\ensuremath{\mathcal{Q}}}
\newcommand\sR{\ensuremath{\mathcal{R}}}
\newcommand\sS{\ensuremath{\mathcal{S}}}
\newcommand\sT{\ensuremath{\mathcal{T}}}
\newcommand\sU{\ensuremath{\mathcal{U}}}
\newcommand\sV{\ensuremath{\mathcal{V}}}
\newcommand\sW{\ensuremath{\mathcal{W}}}
\newcommand\sX{\ensuremath{\mathcal{X}}}
\newcommand\sY{\ensuremath{\mathcal{Y}}}
\newcommand\sZ{\ensuremath{\mathcal{Z}}}
\newcommand\ba{\ensuremath{\mathbf{a}}}
\newcommand\bb{\ensuremath{\mathbf{b}}}
\newcommand\bc{\ensuremath{\mathbf{c}}}
\newcommand\bd{\ensuremath{\mathbf{d}}}
\newcommand\be{\ensuremath{\mathbf{e}}}
\newcommand\bef{\ensuremath{\mathbf{f}}}
\newcommand\bg{\ensuremath{\mathbf{g}}}
\newcommand\bh{\ensuremath{\mathbf{h}}}
\newcommand\bi{\ensuremath{\mathbf{i}}}
\newcommand\bj{\ensuremath{\mathbf{j}}}
\newcommand\bk{\ensuremath{\mathbf{k}}}
\newcommand\bl{\ensuremath{\mathbf{l}}}
\newcommand\bn{\ensuremath{\mathbf{n}}}
\newcommand\bo{\ensuremath{\mathbf{o}}}
\newcommand\bp{\ensuremath{\mathbf{p}}}
\newcommand\bq{\ensuremath{\mathbf{q}}}
\newcommand\br{\ensuremath{\mathbf{r}}}
\newcommand\bs{\ensuremath{\mathbf{s}}}
\newcommand\bt{\ensuremath{\mathbf{t}}}
\newcommand\bu{\ensuremath{\mathbf{u}}}
\newcommand\bv{\ensuremath{\mathbf{v}}}
\newcommand\bw{\ensuremath{\mathbf{w}}}
\newcommand\bx{\ensuremath{\mathbf{x}}}
\newcommand\by{\ensuremath{\mathbf{y}}}
\newcommand\bz{\ensuremath{\mathbf{z}}}
\newcommand\bA{\ensuremath{\mathbf{A}}}
\newcommand\bB{\ensuremath{\mathbf{B}}}
\newcommand\bC{\ensuremath{\mathbf{C}}}
\newcommand\bD{\ensuremath{\mathbf{D}}}
\newcommand\bE{\ensuremath{\mathbf{E}}}
\newcommand\bF{\ensuremath{\mathbf{F}}}
\newcommand\bG{\ensuremath{\mathbf{G}}}
\newcommand\bH{\ensuremath{\mathbf{H}}}
\newcommand\bI{\ensuremath{\mathbf{I}}}
\newcommand\bJ{\ensuremath{\mathbf{J}}}
\newcommand\bK{\ensuremath{\mathbf{K}}}
\newcommand\bL{\ensuremath{\mathbf{L}}}
\newcommand\bM{\ensuremath{\mathbf{M}}}
\newcommand\bN{\ensuremath{\mathbf{N}}}
\newcommand\bO{\ensuremath{\mathbf{O}}}
\newcommand\bP{\ensuremath{\mathbf{P}}}
\newcommand\bQ{\ensuremath{\mathbf{Q}}}
\newcommand\bR{\ensuremath{\mathbf{R}}}
\newcommand\bS{\ensuremath{\mathbf{S}}}
\newcommand\bT{\ensuremath{\mathbf{T}}}
\newcommand\bU{\ensuremath{\mathbf{U}}}
\newcommand\bV{\ensuremath{\mathbf{V}}}
\newcommand\bW{\ensuremath{\mathbf{W}}}
\newcommand\bX{\ensuremath{\mathbf{X}}}
\newcommand\bY{\ensuremath{\mathbf{Y}}}
\newcommand\bZ{\ensuremath{\mathbf{Z}}}
\newcommand\Ba{\ensuremath{\mathbb{a}}}
\newcommand\Bb{\ensuremath{\mathbb{b}}}
\newcommand\Bc{\ensuremath{\mathbb{c}}}
\newcommand\Bd{\ensuremath{\mathbb{d}}}
\newcommand\Be{\ensuremath{\mathbb{e}}}
\newcommand\Bf{\ensuremath{\mathbb{f}}}
\newcommand\Bg{\ensuremath{\mathbb{g}}}
\newcommand\Bh{\ensuremath{\mathbb{h}}}
\newcommand\Bi{\ensuremath{\mathbb{i}}}
\newcommand\Bj{\ensuremath{\mathbb{j}}}
\newcommand\Bk{\ensuremath{\mathbb{k}}}
\newcommand\Bl{\ensuremath{\mathbb{l}}}
\newcommand\Bm{\ensuremath{\mathbb{m}}}
\newcommand\Bn{\ensuremath{\mathbb{n}}}
\newcommand\Bo{\ensuremath{\mathbb{o}}}
\newcommand\Bp{\ensuremath{\mathbb{p}}}
\newcommand\Bq{\ensuremath{\mathbb{q}}}
\newcommand\Br{\ensuremath{\mathbb{r}}}
\newcommand\Bs{\ensuremath{\mathbb{s}}}
\newcommand\Bt{\ensuremath{\mathbb{t}}}
\newcommand\Bu{\ensuremath{\mathbb{u}}}
\newcommand\Bv{\ensuremath{\mathbb{v}}}
\newcommand\Bw{\ensuremath{\mathbb{w}}}
\newcommand\Bx{\ensuremath{\mathbb{x}}}
\newcommand\By{\ensuremath{\mathbb{y}}}
\newcommand\Bz{\ensuremath{\mathbb{z}}}
\newcommand\BA{\ensuremath{\mathbb{A}}}
\newcommand\BB{\ensuremath{\mathbb{B}}}
\newcommand\BC{\ensuremath{\mathbb{C}}}
\newcommand\BD{\ensuremath{\mathbb{D}}}
\newcommand\BE{\ensuremath{\mathbb{E}}}
\newcommand\BF{\ensuremath{\mathbb{F}}}
\newcommand\BG{\ensuremath{\mathbb{G}}}
\newcommand\BH{\ensuremath{\mathbb{H}}}
\newcommand\BI{\ensuremath{\mathbb{I}}}
\newcommand\BJ{\ensuremath{\mathbb{J}}}
\newcommand\BK{\ensuremath{\mathbb{K}}}
\newcommand\BL{\ensuremath{\mathbb{L}}}
\newcommand\BM{\ensuremath{\mathbb{M}}}
\newcommand\BN{\ensuremath{\mathbb{N}}}
\newcommand\BO{\ensuremath{\mathbb{O}}}
\newcommand\BP{\ensuremath{\mathbb{P}}}
\newcommand\BQ{\ensuremath{\mathbb{Q}}}
\newcommand\BR{\ensuremath{\mathbb{R}}}
\newcommand\BS{\ensuremath{\mathbb{S}}}
\newcommand\BT{\ensuremath{\mathbb{T}}}
\newcommand\BU{\ensuremath{\mathbb{U}}}
\newcommand\BV{\ensuremath{\mathbb{V}}}
\newcommand\BW{\ensuremath{\mathbb{W}}}
\newcommand\BX{\ensuremath{\mathbb{X}}}
\newcommand\BY{\ensuremath{\mathbb{Y}}}
\newcommand\BZ{\ensuremath{\mathbb{Z}}}
\newcommand\balpha{\ensuremath{\mbox{\boldmath$\alpha$}}}
\newcommand\bbeta{\ensuremath{\mbox{\boldmath$\beta$}}}
\newcommand\btheta{\ensuremath{\mbox{\boldmath$\theta$}}}
\newcommand\bphi{\ensuremath{\mbox{\boldmath$\phi$}}}
\newcommand\bpi{\ensuremath{\mbox{\boldmath$\pi$}}}
\newcommand\bpsi{\ensuremath{\mbox{\boldmath$\psi$}}}
\newcommand\bmu{\ensuremath{\mbox{\boldmath$\mu$}}}
% Basic
\newcommand\T{\text}
\newcommand\sign{\text{sign}}
\newcommand\tr{\text{tr}}
\newcommand\fig[1]{\begin{center} \includegraphics{#1} \end{center}}
\newcommand\Fig[4]{\begin{figure}[tb] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigTop[4]{\begin{figure}[t] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigStar[4]{\begin{figure*}[tb] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure*}}
\newcommand\aside[1]{\quad\text{[#1]}}
\newcommand\homework[3]{\title{#1} \author{#2} \date{#3} \maketitle}
% Math
\newcommand\argmin{\mathop{\text{argmin}}}
\newcommand\argmax{\mathop{\text{argmax}}}
\newcommand\p[1]{\ensuremath{\left( #1 \right)}} % Parenthesis ()
\newcommand\pb[1]{\ensuremath{\left[ #1 \right]}} % []
\newcommand\pc[1]{\ensuremath{\left\{ #1 \right\}}} % {}
\newcommand\eval[2]{\ensuremath{\left. #1 \right|_{#2}}} % Evaluation
\newcommand\inv[1]{\ensuremath{\frac{1}{#1}}}
\newcommand\half{\ensuremath{\frac{1}{2}}}
\newcommand\R{\ensuremath{\mathbb{R}}} % Real numbers
\newcommand\Z{\ensuremath{\mathbb{Z}}} % Integers
\newcommand\N{\ensuremath{\mathbb{N}}} % Integers
\newcommand\inner[2]{\ensuremath{\left< #1, #2 \right>}} % Inner product
\newcommand\mat[2]{\ensuremath{\left(\begin{array}{#1}#2\end{array}\right)}} % Matrix
\newcommand\eqn[1]{\begin{eqnarray} #1 \end{eqnarray}} % Equation (array)
\newcommand\eqnl[2]{\begin{eqnarray} \label{eqn:#1} #2 \end{eqnarray}} % Equation (array) with label
\newcommand\eqdef{\ensuremath{\stackrel{\rm def}{=}}} % Equal by definition
%\newcommand{\1}{\mathbb{I}} % Indicator (don't use \mathbbm{1} because bbm is not TrueType though)
\newcommand{\1}{\ensuremath{\mathbbm{1}}}
\newcommand{\bone}{\mathbf{1}} % for vector one
\newcommand{\bzero}{\mathbf{0}} % for vector zero
\newcommand\refeqn[1]{(\ref{eqn:#1})}
\newcommand\refeqns[2]{(\ref{eqn:#1}) and (\ref{eqn:#2})}
\newcommand\refchp[1]{Chapter~\ref{chp:#1}}
\newcommand\refsec[1]{Section~\ref{sec:#1}}
\newcommand\refsecs[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand\reffig[1]{Figure~\ref{fig:#1}}
\newcommand\reffigs[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand\reffigss[3]{Figures~\ref{fig:#1},~\ref{fig:#2}, and~\ref{fig:#3}}
\newcommand\reffigsss[4]{Figures~\ref{fig:#1},~\ref{fig:#2},~\ref{fig:#3}, and~\ref{fig:#4}}
\newcommand\reftab[1]{Table~\ref{tab:#1}}
\newcommand\refapp[1]{Appendix~\ref{sec:#1}}
\newcommand\refthm[1]{Theorem~\ref{thm:#1}}
\newcommand\refthms[2]{Theorems~\ref{thm:#1} and~\ref{thm:#2}}
\newcommand\reflem[1]{Lemma~\ref{lem:#1}}
\newcommand\reflems[2]{Lemmas~\ref{lem:#1} and~\ref{lem:#2}}
\newcommand\refprop[1]{Proposition~\ref{prop:#1}}
\newcommand\refdef[1]{Definition~\ref{def:#1}}
\newcommand\refcor[1]{Corollary~\ref{cor:#1}}
\newcommand\refalg[1]{Algorithm~\ref{alg:#1}}
\newcommand\Chapter[2]{\chapter{#2}\label{chp:#1}}
\newcommand\Section[2]{\section{#2}\label{sec:#1}}
\newcommand\Subsection[2]{\subsection{#2}\label{sec:#1}}
\newcommand\Subsubsection[2]{\subsubsection{#2}\label{sec:#1}}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
% Probability
\newcommand\cv{\ensuremath{\to}} % Convergence
\newcommand\cvL{\ensuremath{\xrightarrow{\mathcal{L}}}} % Convergence in law
\newcommand\cvd{\ensuremath{\xrightarrow{d}}} % Convergence in distribution
\newcommand\cvP{\ensuremath{\xrightarrow{P}}} % Convergence in probability
\newcommand\cvas{\ensuremath{\xrightarrow{a.s.}}} % Convergence almost surely
\newcommand\eqdistrib{\ensuremath{\stackrel{d}{=}}} % Equal in distribution
\newcommand\E[1]{\ensuremath{\mathbb{E}{\left[#1\right]}}} % Expectation
\newcommand\Ex[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}} % Expectation
\newcommand\var{\ensuremath{\text{var}}} % Variance
\newcommand\cov{\ensuremath{\text{cov}}} % Covariance
\newcommand\diag{\ensuremath{\text{diag}}} % Diagnonal matrix
\newcommand\cE[2]{\ensuremath{\E \left( #1 \mid #2 \right)}} % Conditional expectation
\newcommand\KL[2]{\ensuremath{\T{KL}\left( #1 \,||\, #2 \right)}} % KL-divergence
\newcommand\D[2]{\ensuremath{\bD\left( #1 \,||\, #2 \right)}} % KL-divergence

% Utilities
\newcommand\lte{\leq}
\newcommand\gte{\geq}
\newcommand\lone[1]{\ensuremath{\|#1\|_1}}
\newcommand\ltwo[1]{\ensuremath{\|#1\|_2^2}}
\newcommand\naive{na\"{\i}ve}
\newcommand\Naive{Na\"{\i}ve}

% Debug
\usepackage{color}
\newcommand{\hl}[2]{\colorbox{#2}{#1}}
\newcommand{\hly}[1]{\hl{yellow}{#1}}
\def\todo#1{\hl{{\bf TODO:} #1}{yellow}}
\def\needcite{\hl{{$^{\tt\small[citation\ needed]}$}}{blue}}
\def\needfig{\hl{Figure X}{green}}
\def\needtab{\hl{Table Y}{green}}
\def\note#1{\hl{{\bf NOTE:} #1}{yellow}}
\def\dome{\hl{{\bf TODO:} write me!}{yellow}}


==> todos.tex <==
\section{TODO}

\subsection{Arun}

\begin{itemize}
  \item I don't like that "money" and "time" are explicit variables in the loss function, mainly because it seems too concrete for abstract math. We can choose an specific loss function at a later time dependent on those parameters. I might yet come around to this notation.
\end{itemize}

